Easy Guided Decoding in Providing Suggestions for Interactive Machine Translation

Machine translation technology has made great progress in recent years, but it cannot guarantee error free results. Human translators perform post editing on machine translations to correct errors in the scene of computer aided translation. In favor of expediting the post editing process, many works have investigated machine translation in interactive modes, in which machines can automatically refine the rest of translations constrained by human's edits. Translation Suggestion (TS), as an interactive mode to assist human translators, requires machines to generate alternatives for specific incorrect words or phrases selected by human translators. In this paper, we utilize the parameterized objective function of neural machine translation (NMT) and propose a novel constrained decoding algorithm, namely Prefix Suffix Guided Decoding (PSGD), to deal with the TS problem without additional training. Compared to the state of the art lexically constrained decoding method, PSGD improves translation quality by an average of $10.87$ BLEU and $8.62$ BLEU on the WeTS and the WMT 2022 Translation Suggestion datasets, respectively, and reduces decoding time overhead by an average of 63.4% tested on the WMT translation datasets. Furthermore, on both of the TS benchmark datasets, it is superior to other supervised learning systems trained with TS annotated data.

==> related_works.tex <==
\section {Related Work}

Some related works have been explored in computer-aided translation. \citet{wuebker-etal-2016-models} and \citet{knowles-koehn-2016-neural} proposed an NMT Interactive Translation Prediction (ITP) method, focusing on how to complete partial translations of words or phrases given a prefix. \citet{santy2019inmt} further presented an interactive translation system conditioned on hints from translators on low-resource language pairs. These post-editing applications paid attention to the overall performance but ignored the performance on suggestion parts. \citet{yang2021wets} proposed the translation suggestion benchmark, and extensively took the performance of the suggested words or phrases into consideration, which would be highly appreciated in practical applications. 

As for the constrained decoding algorithms, previous works tried to support lexical constraints when decoding with generative models. \citet{hokamp-liu-2017-lexically} introduced Grid Beam Search (GBS), modifying the inference procedure to promise the hard lexical constraints without iterating model parameters on any additional training data. \citet{anderson-etal-2017-guided} used the constrained beam search (CBS) for object captioning in an image, which extends beam search by marking the status of the constraints with a finite-state machine. However, these two methods have linear and exponential computational complexities in the number of constraints respectively. 

\citet{post-vilar-2018-fast} proposed Dynamic Beam Allocation (DBA) with $\mathcal{O}(1)$ computational complexities in the number of provided constraints. It tries to allocate slots in the beam to ensure a fixed-sized beam during generations regardless of the number of constraints. Another improved work, VDBA, was proposed by \citet{hu-etal-2019-improved}, which accelerates decoding by using dynamic vectorization for batch decoding. Besides, VDBA uses a multi-state try to avoid certain corners in DBA to further improve the translation quality. Considering the advantages of VDBA \citep{hu-etal-2019-improved}, we mainly regard it as the comparison algorithm. 
